Osiris: A Systolic Approach to Accelerating Fully Homomorphic Encryption

In this paper we show how fully homomorphic encryption (FHE) can be accelerated using a systolic architecture. We begin by analyzing FHE algorithms and then develop systolic or systolic-esque units for each major kernel. Connecting units is challenging due to the different data access and computational patterns of the kernels. We overcome this by proposing a new data tiling technique that we name limb interleaving. Limb interleaving creates a common data input/output pattern across all kernels that allows the entire architecture, named Osiris, to operate in lockstep. Osiris is capable of processing key-switches, bootstrapping, and full neural network inferences with high utilization across a range of FHE parameters. To achieve high performance, we propose a new giant-step centric (GSC) dataflow that efficiently maps state-of-the-art FHE matrix-vector product algorithms onto Osiris by optimizing for reuse and parallelism. Our evaluation of Osiris shows it outperforms the prior state-of-the-art accelerator on all standard benchmarks.

==> 07-hoisting.tex <==

\noindent\textbf{On-the-fly Limb Extension:} We adopt the on-the-fly limb extension (OF-Limb) technique originally proposed for use in hardware acceleration by ARK \cite{ark} to improve arithmetic intensity. 
OF-Limb uses a single precomputed limb ($q_0$) of the plaintext diagonal (coefficient representation) to generate all other limbs.
The optimization saves significant off-chip communication at the cost of additional computation to generate them on-chip.
We can generate any $i$'th limb from this $q_0$-limb through the following equation:
\begin{equation*}
    [\mathtt{P}]_{q_i} = \mathsf{NTT}([\mathtt{P_{coeff}}]_{q_0}) \hspace{-4px} \mod q_i
\end{equation*}

Therefore, OF-Limb is performed with $\mathsf{Osiris}$’ MDC units. 
We use this technique to generate \textit{all} plaintext diagonals in the matrix-vector products in bootstrapping and in the linear and convolutional layers of neural networks.

\vspace{2px}

\noindent \textbf{Giant-Step Centric Dataflow:} To maximize the arithmetic intensity of matrix-vector products that use the baby-step giant-step (BSGS) algorithm, we propose a novel \textit{giant-step centric} (GSC) dataflow. 
Recall from Algorithm \ref{alg:bsgs} that the BSGS algorithm reduces the number of ciphertext rotations in a matrix-vector product with $n$ non-zero diagonals from $n$ to $n_1+n_2$, where $n_1 n_2=n$. 
Broadly, the goal of the GSC dataflow is to mask the latency of loading each baby-step rotation key with diagonal generation using OF-Limb. We visualize this dataflow alongside a high-level overview of the double-hoisting algorithm in Figure \ref{fig:gsc-dataflow} using the same matrix-vector product introduced in Section \ref{sect:mv-products}.  

We highlight three features of Figure \ref{fig:gsc-dataflow}. First, rotations to the \textit{same} input ciphertext share a common $\mathsf{Decompose}$ output. Therefore, we can perform this computation only once, \textit{hoisting} it out and reusing its result for all $n_1$ baby-step rotations. Similarly, Bossuat et al. \cite{bossuat} show that the $\mathsf{ModDown}$ operation commutes with addition, e.g., $\sum_i \mathsf{ModDown(ct}_i\mathsf{)} = \mathsf{ModDown}(\sum_i \mathsf{ct}_i)$. Therefore, a similar \textit{second} level of hoisting can be performed when summing all giant steps. 
We cache the $\mathsf{Decompose}$ output to leverage its significant reuse. 

Second, we use OF-Limb to generate the limbs of \textit{all} plaintext matrix diagonals. Since each baby-step rotation key contributes to $n_2$ partial products, we naturally group generated diagonals into $n_1$ sets of $n_2$ diagonals to minimize off-chip memory accesses. While our MDC units are generating the current set of $n_2$ matrix diagonals, we load the next baby-step rotation key on-chip and use our Hadamard and Automorphism units to prepare the ciphertext’s next baby-step rotation. Thus, if the latency of fetching a rotation key is less than the latency of generating $n_2$ plaintext diagonals, then DRAM accesses are completely overlapped.
We deliberately size $\mathsf{Osiris}$' width with this step in mind. 


Third, since we iteratively generate each set of $n_2$ partial products, we can accumulate these products to reserved on-chip SRAM locations, reducing the size of our working set. When the ideal number of giant steps exceeds what can be stored on-chip, we find it more efficient to simply reduce the number of giant steps in the BSGS algorithm rather than send partial products off-chip. Since each giant step rotates a \textit{unique} ciphertext, we cannot hoist out a common $\mathsf{Decompose}$ step. Consequently, giant steps are more expensive than baby steps, and the optimal ratio of $n_1 / n_2$ is large, often varying between $8$ and $16$ \cite{bossuat}. 
We set the maximum number of giant steps held on-chip to be $n_2=4$ in the highest multiplicative level matrix-vector products in bootstrapping.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/gcs-dataflow.pdf}
    \caption{Visualizing how the GSC dataflow masks rotation key DRAM accesses with on-the-fly limb extension (OF-Limb) using the BSGS example introduced in Figure \ref{fig:bsgs}.}
    \label{fig:gsc-dataflow}
    \vspace{5px}
\end{figure}

\vspace{2px}
\noindent\textbf{Architecting Osiris:} Figure \ref{fig:osiris-arch} presents the full $\mathsf{Osiris}$ architecture. An important distinction between $\mathsf{Osiris}$ and prior FHE accelerators is that we dedicate \textit{separate} units to each step of the $\mathsf{ModChange}$ ($\mathsf{INTT}\rightarrow \mathsf{BConv} \rightarrow \mathsf{NTT}$) routine. This difference is motivated by our choice to feed limbs through $\mathsf{Osiris}$ in an \textit{interleaved} fashion. Recall from Section \ref{sect:osiris-arch} that interleaving resolves the differences between the desired input order of I/NTT and $\mathsf{BConv}$ and enables the units to operate together in lockstep. Therefore, when mapped onto $\mathsf{Osiris}$, it is useful to view the $\mathsf{ModChange}$ operation as a single, macro-pipeline with a throughput of one output limb every $\sfrac{N}{p}$ cycles. 

We also note that while the BSGS algorithm reduces the number of ciphertext rotations in matrix-vector products, it does not reduce the number of plaintext diagonal multiplications. When the number of non-zero diagonals is large, a significant fraction of end-to-end latency comes from OF-Limb. To mitigate this bottleneck, we leverage the bidirectional nature of pipelined NTT architectures to reverse the direction of our $\mathsf{ModChange}$'s MDC INTT unit for the duration of OF-Limb. Since OF-Limb generates diagonals through repeated NTTs, the INTT unit would otherwise be left idle. This strategy doubles the throughput of OF-Limb, and we place Hadamard units on each side of $\mathsf{Osiris}$ to generate and accumulate partial products.


